Modeling Causal Mechanisms with Diffusion Models for Interventional and Counterfactual Queries

We consider the problem of answering observational, interventional, and counterfactual queries in a causally sufficient setting where only observational data and the causal graph are available. Utilizing the recent developments in diffusion models, we introduce diffusion-based causal models (DCM) to learn causal mechanisms, that generate unique latent encodings. These encodings enable us to directly sample under interventions and perform abduction for counterfactuals. Diffusion models are a natural fit here, since they can encode each node to a latent representation that acts as a proxy for exogenous noise. Our empirical evaluations demonstrate significant improvements over existing state-of-the-art methods for answering causal queries. Furthermore, we provide theoretical results that offer a methodology for analyzing counterfactual estimation in general encoder-decoder models, which could be useful in settings beyond our proposed approach.

==> tex_files/dcm_arxiv.tex <==
In this section, we present our \DCM approach for modeling the SCMs and to answer causal queries. We first explain the construction and the training process of a \DCM, and then explain how the model can be used for answering various causal queries. 
% Given a causal graph $\cG$ over endogenous variables $(X_1,\ldots,X_K)$, we may topologically sort the graph and relabel the nodes, implying $j< i$ for all $j\in \pa_i$, and assume $X_i\in\R^{d_i}$. 
We start with some notations.
\begin{CompactItemize}
     \item Define $Z_i^t$ to be the $i$th endogenous node value at diffusion step $t$ of the \textit{forward} implicit diffusion process (Eq.~\eqref{eq: forward implicit diffusion}), and let $Z_i\coloneqq Z_i^T$. 
    \item Define $\hat X_i^t$ to be $i$th endogenous node value at diffusion step $t$ of the \textit{reverse} implicit diffusion process (Eq.~\eqref{eq: ddim reverse}), and let $\hat X_i\coloneqq \hat X_i^0$.   
\end{CompactItemize}

\noindent\textbf{Training a \DCM.} We train a diffusion model for \textit{each node}, taking denoised parent values as input. The parent values can be interpreted as additional covariates to the model, where one may choose to use classifier free guidance to incorporate the covariates \citep{ho2021classifierfree}. Empirically, we find that simply concatenating the covariates results in better performance than classifier free guidance.
% and provide theoretical intuition for this phenomenon in Theorem \ref{thm: cf theory} and Section \ref{subsec: model implementation}.



% determining the counterfactual outcome of a particular variable $X_j$ subject to an intervention on another variable $X_{j'}$ then the problem becomes simple. For example, we can take any backdoor adjustment set $A$ relative to $(X_j,X_{j'})$ and simply reduce the graph to these variables. 

We use the $\ep_\theta$ parametrization for the diffusion model from \citet{ddpm}, representing the diffusion model for node $i$ as $\ep_\theta^i(X, X_{\pa_i},t)$. The complete training procedure presented in Algorithm \ref{algo: DCM training} is only slightly modified from the usual training procedure, with the additions of the parents as covariates and training a diffusion model for each node. Since the generative models learned for generation of different endogenous nodes do not affect training of each other,
these models may be trained in parallel. Our final DCM model is just a combination of these $K$ trained diffusion models $\ep_\theta^1,\dots,\ep_\theta^K$.

% We focus on learning a single generative model (and a corresponding inference mechanism) for the generation of the
% endogenous node Y , given its parents T in the causal graph (T → Y )
\begin{algorithm}[!ht]
    \caption{\DCM Training}
    \label{algo: DCM training}
    \textbf{Input:} Distribution $Q$, scale factors $\{\alpha_t\}_{t=1}^T$, causal DAG $\cG$ with node $i$ represented by $X_i$
    \begin{algorithmic}[1]
        \WHILE{not converged}
        \STATE Sample $X^0\sim Q$
        \FOR{$i=1,\ldots,K$}
            \STATE $t\sim \mathrm{Unif}[\{1,\ldots,T\}]$
            \STATE $\ep\sim\cN(0,I_{d_i})$ \hfill\Comment{$d_i$ is the dimension of $X_i$}
            \STATE Update parameters of node $i$'s diffusion model $\ep_\theta^i$, by minimizing the following loss:   
 \hspace*{1.75in} $\|\ep-\ep_\theta^i(\sqrt{\alpha_t}X_i^0+\sqrt{1- \alpha_t}\ep,X_{\pa_i}^0,t)\|_2^2$    (based on Eq.\ \eqref{eq: simple objective})  
        \ENDFOR
         \ENDWHILE
    \end{algorithmic}
\end{algorithm}

We use all the variables $(X_1,\ldots,X_K)$ for the training procedure, because a priori, we do not assume anything on the possible causal queries, i.e., we allow for all possible target variables, intervened variables, etc. However, if we are only interested in some pre-defined set of queries, then the graph could be reduced accordingly. For example, if we are only interested in counterfactual estimate of a particular node with respect to an intervention of a predecessor, one can simply reduce it to a subgraph containing the target node, the intervened node and a backdoor adjustment set (e.g., the ancestors of the intervened node). This then reduces to only learning a single diffusion model. 

\noindent\textbf{Encoding and Decoding Steps with \DCM.} With a \DCM, the encoding (resp.\ decoding) process is identical to the DDIM encoding (resp.\ decoding) process except we include the  parent values as additional covariates.
Let us focus on a node $i \in [K]$ (same process is repeated for each node $i$). The encoding process takes $X_i$ and its parent values $X_{\pa_i}$ as input and maps it to a latent variable $Z_i$. The decoding process takes $Z_i$ and $X_{\pa_i}$ as input to construct $\hat{X}_i$ (an approximation of $X_i$). Formally, using the forward implicit diffusion process in Eq.\ \eqref{eq: forward implicit diffusion}, given a sample $X_i$, we encode a unique latent variable $Z_i:=Z_i^T$, using the recursive formula 
\begin{align} \label{eq:1}
  Z^{t+1}_i := \sqrt{\frac{\alpha_{t+1}}{\alpha_t}}Z^t_i + \ep_\theta^i(Z^t_i,X_{\pa_i},t)\left(\sqrt{1-\alpha_{t+1}}-\sqrt{\frac{\alpha_{t+1}(1-\alpha_t)}{\alpha_t}}\right), \forall t = 0,..,T-1,  
\end{align}
where $Z_i^0 :=X_i$.
The latent variable $Z_i$ acts as a proxy for the exogenous noise $U_i$.
% For example, assume $X_i=f(X_{\pa_i})+U_i$ where $X_i$ and $U_i$ are scalars. We would like to have $Z_i=\tilde q(U_i)$ for some invertible function $\tilde q$. However, in practice, we do not need the latent variable $Z_i$ to exactly satisfy this, and our diffusion model at node $i$ learns to capture a representation of the exogenous noise $U_i$. Also by construction, $Z_i$ and $X_i$ have the same dimension.\!\footnote{As we will see through our theoretical results in \cref{thm: cf theory,thm: multivariate cf theory}, this is in fact a desirable property.}
% which allows DCM to capture the maximum effective dimensionality of $U_i$
% \marginpar{Need some clarification on what is $Z_i$: $U_i$ is a random variable, are they of different dimension?
% PC: Added more details, I am not sure how clear the effective dimensionality is}
% \marginpar{No, that is not clear. Plus, why is this even important for capturing info about $U_i$?}
% \marginpar{It is important to capture information about $U_i$ since this is what you use in the decoding process for interventional and counterfactual inference.}
Using the reverse implicit diffusion process from DDIM in Eq.\ \eqref{eq: ddim reverse}, given a latent vector $Z_i$ we obtain a deterministic decoding $\hat X_i:=\hat{X}_i^0$, using the recursive formula
\begin{align} \label{eq:2}
\hat X^{t-1}_i := \sqrt{ \frac{\alpha_{t-1}}{\alpha_t}}\hat X^t_i -\ep_\theta^i( \hat X_i^t,X_{\pa_i},t)  \left(\sqrt{\frac{\alpha_{t-1}(1-\alpha_{t})}{\alpha_t}}-\sqrt{1-\alpha_{t-1}}\right),  \forall t = T,..,1,
\end{align}
where $\hat{X}^T:=Z_i$. In the following, we use $\enc_i(X_i,X_{\pa_i})$ and $\dec_i(Z_i,X_{\pa_i})$ to denote the encoding and decoding functions for node $i$ defined in Eqns.~\eqref{eq:1} and~\eqref{eq:2} respectively. See Algorithms \ref{algo: DCM encoding} and \ref{algo: DCM decoding}  for detailed pseudocodes.
 
% and decode the graph in topological order.


% We define $\enc_i(X_i,X_{\pa_i})$ and $\dec_i(Z_i,X_{\pa_i})$ to be the implicit encoding and decoding functions for node $i$ defined in Eqns.~\eqref{eq: forward implicit diffusion} and~\eqref{eq: ddim reverse} respectively when applied recursively $T$ times, explicitly   respectively.


 


\noindent\textbf{Answering Causal Queries with a Trained \DCM.}  We now describe how a trained \DCM model can be used for (approximately) answering causal queries. Answering observational and interventional queries require sampling from the observational and the interventional distribution respectively. With counterfactuals, a query is at the unit level, where the structural assignments are changed, but the exogenous noise is identical to that of the observed datum.
% For interventional and counterfactual queries, consider a set of intervened variables $X_{\cI} \subseteq \mathbf{X}$ (for $\cI \subseteq [K]$)  and values $\gamma \in \R^{|\cI|}$, where $\doo(X_\cI:=\gamma)\coloneqq\{\doo(X_i:=\gamma_i)\}_{i\in\cI}$. 

\textbf{(a) Generating Samples for Observational/Interventional Queries.} Samples from a \DCM model that approximates the interventional distribution $p(\mathbf{X}\mid \doo(X_\cI:=\gamma))$ can be generated as follows. For an intervened node $i$ with intervention $\gamma_i$, the sampled value is always the intervention value, therefore we generate $\hat X_i:=\gamma_i$. 
% For root nodes, we sample $\hat X_i$ from the empirical distribution of the training set. 
For a non-intervened node $i$, assume by induction we have the generated parent values $\hat X_{\pa_i}$. To generate $\hat X_i$, we first sample the latent vector $Z_i\sim\cN(0,I_{d_i})$ where $d_i$ is the dimension of $X_i$. Then taking $Z_i$ as the noise for node $i$, we compute $\hat X_i:=\dec_i(Z_i,\hat X_{\pa_i})$ as the generated sample value for node $i$. This value $\hat X_i$ is then used as the parent value for the children of node $i$. Samples from a \DCM model that approximates the observational distribution $p(\mathbf{X})$ can be generated by setting $\cI=\emptyset$ (see Algorithm~\ref{algo: cdm intervention sampling}).

\begin{algorithm}[!h]
    \caption{Observational/Interventional Sampling}
    \label{algo: cdm intervention sampling}
    \textbf{Input:} Intervention set $\cI$ with values $\gamma$ ($I = \emptyset$ for observational sampling)
    \begin{algorithmic}[1]
        \FOR{$i=1,\ldots,K$} \hfill\COMMENT{in topological order}
            \STATE $Z_i \sim\cN(0,I_{d_i})$
            \IF{$i\in \cI$}
            \STATE $\hat X_i \leftarrow \gamma_i$
            % \ELSIF{$i$ is a root node}
            % \STATE $\hat X_i\sim \mathcal{E}_i$ where $\mathcal{E}_i$ is the empirical distribution of the node $X_i$
            \ELSE
            \STATE $\hat X_i \leftarrow \dec_i(Z_i,\hat X_{\pa_i})$
            \ENDIF
        \ENDFOR
    \STATE Return $\hat X := (\hat X_1,\dots,\hat X_K)$
    \end{algorithmic}
\end{algorithm}




\begin{algorithm}[!h]
    \caption{Counterfactual Inference}
    \label{algo: DCM counterfactual inference}
    \textbf{Input:} Intervention set $\cI$ with values $\gamma$, factual sample~$x^\fact := (x_1^\fact,\dots,x_K^\fact)$
    \begin{algorithmic}[1]
     \FOR{$i=1,\ldots,K$} \hfill\COMMENT{in topological order}
        \IF{$i\in \cI$}
            \STATE $\hat x^\cf_i \leftarrow \gamma_i$
            \ELSIF{$i$ is not a descendant of any intervened node in $\cI$}
            \STATE $\hat x^\cf_i \leftarrow x^\fact_i$
            \ELSE
            \STATE  $z^\fact_i\leftarrow \enc_i(x^\fact_i,x_{\pa_i}^\fact)$ \hfill \Comment{abduction step}
            \STATE $\hat x^\cf_i \leftarrow \dec_i(z_i,\hat x_{\pa_i})$ \hfill\Comment{action and prediction steps}
            \ENDIF
        \ENDFOR
     \STATE Return $\hat x^\cf := (\hat x^\cf_1,\dots,\hat x^\cf_K)$
    \end{algorithmic}
\end{algorithm}

\textbf{(b) Counterfactual Queries.} 
Consider a factual observation $x^\fact:=(x_1^\fact,\dots,x_K^\fact)$ and interventions on a set of nodes $\cI$ with values $\gamma$. We use a \DCM model to construct a counterfactual estimate $\hat{x}^\cf$ as follows. The counterfactual estimate only differs from the factual value on intervened nodes or descendants of an intervened node. Similarly to interventional queries, for each intervened node $i \in \cI$, $\hat x_i^\cf:=\gamma_i$. For each non-intervened node $i$ that is a descendant of any intervened node, assume by induction that we have the generated counterfactual estimates $\hat x_{\pa_i}^\cf$. To obtain $\hat x_i^\cf$, we first define the estimated factual noise as $\hat z_i^\fact:=\enc_i(x_i^\fact, x_{\pa_i}^\fact)$. Then we  generate our counterfactual estimate by using $\hat z_i^\fact$ as the noise for node $i$, by decoding, $\hat x_i^\cf := \dec_i(\hat z_i^\fact,\hat x_{\pa_i}^\cf)$ (see Algorithm \ref{algo: DCM counterfactual inference}). 

Note that with $x^\fact$, we assumed full observability,\!\footnote{This is a common assumption in literature also made in all the related work e.g.,~\citep{vaca,carefl,pawlowski2020deep}.} since because Algorithm \ref{algo: DCM counterfactual inference} produces a counterfactual estimate for each node. However, when intervening on $X_\cI$ and if the only quantity of interest is  counterfactual on some $X^\star$, then you only need factual samples from $\{X_i:X_i\text{ is on a path from } X_{\cI} \to X^\star\}$~\citep{sahanoise}. In practice, this could be further relaxed by imputing for missing data, which is beyond the scope of this work.
% \textcolor{blue}{However, if we are only interested in counterfactual estimate at some node $\hat X_i^\cf$, all we need is for $X^\fact$ to contain values of $X_i$ and its ancestors. }
% \marginpar{To check this, can we set $Z_i$'s to $I_{d_i}$?}
% \textcolor{blue}{However, as is evident from Algorithm \ref{algo: DCM counterfactual inference},  if we are only interested in counterfactual estimate at some node $\hat X_i^\cf$, all we need is for $X^\fact$ to contain both $X_i^\fact$ and $X_{\pa_i}^\fact$ as we will see in the next section. In practice, even this could be relaxed by imputing for missing data, which is beyond the scope of this work.}
% \textcolor{red}{This does not seem to be true, you need $X_i^\fact$, $X_{\pa_i}^\fact$, and $\hat X_{\pa_i}$, which implicitly contains all of the upstream values as well.}
% \marginpar{How about this?}



==> tex_files/dcm_icml_workshop.tex <==
In this section, we present our \DCM approach for modeling the SCMs and to answer causal queries. We first explain the construction and the training process of a \DCM, and then explain how the model can be used for answering various causal queries. 
% Given a causal graph $\cG$ over endogenous variables $(X_1,\ldots,X_K)$, we may topologically sort the graph and relabel the nodes, implying $j< i$ for all $j\in \pa_i$, and assume $X_i\in\R^{d_i}$. 
We start with some notations.
\begin{CompactItemize}
     \item Define $Z_i^t$ to be the $i$th endogenous node value at diffusion step $t$ of the \textit{forward} implicit diffusion process (Eq.~\eqref{eq: forward implicit diffusion}), and let $Z_i\coloneqq Z_i^T$. 
    \item Define $\hat X_i^t$ to be $i$th endogenous node value at diffusion step $t$ of the \textit{reverse} implicit diffusion process (Eq.~\eqref{eq: ddim reverse}), and let $\hat X_i\coloneqq \hat X_i^0$.   
\end{CompactItemize}

\textbf{Training a \DCM.} We train a diffusion model for \textit{each node}, taking denoised parent values as input. The parent values can be interpreted as additional covariates to the model, where one may choose to use classifier free guidance to incorporate the covariates \citep{ho2021classifierfree}. Empirically, we find that simply concatenating the covariates results in better performance than classifier free guidance.
% and provide theoretical intuition for this phenomenon in Theorem \ref{thm: cf theory} and Section \ref{subsec: model implementation}.



% determining the counterfactual outcome of a particular variable $X_j$ subject to an intervention on another variable $X_{j'}$ then the problem becomes simple. For example, we can take any backdoor adjustment set $A$ relative to $(X_j,X_{j'})$ and simply reduce the graph to these variables. 

We use the $\ep_\theta$ parametrization for the diffusion model from \citet{ddpm}, representing the diffusion model for node $i$ as $\ep_\theta^i(X, X_{\pa_i},t)$. The complete training procedure presented in Algorithm \ref{algo: DCM training} is only slightly modified from the usual training procedure, with the additions of the parents as covariates and training a diffusion model for each node. Since the generative models learned for generation of different endogenous nodes do not affect training of each other,
these models may be trained in parallel. Our final DCM model is just a combination of these $K$ trained diffusion models $\ep_\theta^1,\dots,\ep_\theta^K$.

% We focus on learning a single generative model (and a corresponding inference mechanism) for the generation of the
% endogenous node Y , given its parents T in the causal graph (T → Y )
\begin{algorithm}[!ht]
    \caption{\DCM Training}
    \label{algo: DCM training}
    \textbf{Input:} Distribution $Q$, scale factors $\{\alpha_t\}_{t=1}^T$, causal DAG $\cG$ with node $i$ represented by $X_i$
    \begin{algorithmic}[1]
        \WHILE{not converged}
        \STATE Sample $X^0\sim Q$
        \FOR{$i=1,\ldots,K$}
            \STATE $t\sim \mathrm{Unif}[\{1,\ldots,T\}]$
            \STATE $\ep\sim\cN(0,I_{d_i})$ \hfill\COMMENT{$d_i$ is the dimension of $X_i$}
            \STATE Update parameters of node $i$'s diffusion model $\ep_\theta^i$, by minimizing the following loss (from Eq.\ \eqref{eq: simple objective}):   \\
 $\|\ep-\ep_\theta^i(\sqrt{\alpha_t}X_i^0+\sqrt{1- \alpha_t}\ep,X_{\pa_i}^0,t)\|_2^2$   
        \ENDFOR
         \ENDWHILE
    \end{algorithmic}
\end{algorithm}

We use all the variables $(X_1,\ldots,X_K)$ for the training procedure, because a priori, we do not assume anything on the possible causal queries, i.e., we allow for all possible target variables, intervened variables, etc. However, if we are only interested in some pre-defined set of queries, then the graph could be reduced accordingly. For example, if we are only interested in counterfactual estimate of a particular node with respect to an intervention of a predecessor, one can simply reduce it to a subgraph containing the target node, the intervened node and a backdoor adjustment set (e.g., the ancestors of the intervened node). This then reduces to only learning a single diffusion model. 

\textbf{Encoding and Decoding Steps with \DCM.} With a \DCM, the encoding (resp.\ decoding) process is identical to the DDIM encoding (resp.\ decoding) process except we include the  parent values as additional covariates.
Let us focus on a node $i \in [K]$ (same process is repeated for each node $i$). The encoding process takes $X_i$ and its parent values $X_{\pa_i}$ as input and maps it to a latent variable $Z_i$. The decoding process takes $Z_i$ and $X_{\pa_i}$ as input to construct $\hat{X}_i$ (an approximation of $X_i$). Formally, using the forward implicit diffusion process in Eq.\ \eqref{eq: forward implicit diffusion}, given a sample $X_i$, we encode a unique latent variable $Z_i:=Z_i^T$, using the recursive formula 
\begin{equation} \label{eq:1}
\begin{split}
Z^{t+1}_i &\coloneqq \sqrt{\frac{\alpha_{t+1}}{\alpha_t}}Z^t_i + \ep_\theta^i(Z^t_i,X_{\pa_i},t)\;\cdot\\
  &\left(\sqrt{1-\alpha_{t+1}}-\sqrt{\frac{\alpha_{t+1}(1-\alpha_t)}{\alpha_t}}\right),   
\end{split}
\end{equation}  
for all $t = 0,\ldots ,T-1$, where $Z_i^0 :=X_i$.
The latent variable $Z_i$ acts as a proxy for the exogenous noise $U_i$.
% For example, assume $X_i=f(X_{\pa_i})+U_i$ where $X_i$ and $U_i$ are scalars. We would like to have $Z_i=\tilde q(U_i)$ for some invertible function $\tilde q$. However, in practice, we do not need the latent variable $Z_i$ to exactly satisfy this, and our diffusion model at node $i$ learns to capture a representation of the exogenous noise $U_i$. Also by construction, $Z_i$ and $X_i$ have the same dimension.\!\footnote{As we will see through our theoretical results in \cref{thm: cf theory,thm: multivariate cf theory}, this is in fact a desirable property.}
% which allows DCM to capture the maximum effective dimensionality of $U_i$
% \marginpar{Need some clarification on what is $Z_i$: $U_i$ is a random variable, are they of different dimension?
% PC: Added more details, I am not sure how clear the effective dimensionality is}
% \marginpar{No, that is not clear. Plus, why is this even important for capturing info about $U_i$?}
% \marginpar{It is important to capture information about $U_i$ since this is what you use in the decoding process for interventional and counterfactual inference.}
Using the reverse implicit diffusion process from DDIM in Eq.\ \eqref{eq: ddim reverse}, given a latent vector $Z_i$ we obtain a deterministic decoding $\hat X_i:=\hat{X}_i^0$, using the recursive formula
\begin{equation} \label{eq:2}
\begin{split}
\hat X^{t-1}_i &\coloneqq \sqrt{ \frac{\alpha_{t-1}}{\alpha_t}}\hat X^t_i -\ep_\theta^i( \hat X_i^t,X_{\pa_i},t)  \;\cdot\\
&\left(\sqrt{\frac{\alpha_{t-1}(1-\alpha_{t})}{\alpha_t}}-\sqrt{1-\alpha_{t-1}}\right),  
\end{split}
\end{equation}
for all $t=T,\ldots,1$ where $\hat{X}^T:=Z_i$. In the following, we use $\enc_i(X_i,X_{\pa_i})$ and $\dec_i(Z_i,X_{\pa_i})$ to denote the encoding and decoding functions for node $i$ defined in Eqns.~\eqref{eq:1} and~\eqref{eq:2} respectively. See Algorithms \ref{algo: DCM encoding} and \ref{algo: DCM decoding}   (Appendix~\ref{app: encdec}) for detailed pseudocodes.
 
% and decode the graph in topological order.


% We define $\enc_i(X_i,X_{\pa_i})$ and $\dec_i(Z_i,X_{\pa_i})$ to be the implicit encoding and decoding functions for node $i$ defined in Eqns.~\eqref{eq: forward implicit diffusion} and~\eqref{eq: ddim reverse} respectively when applied recursively $T$ times, explicitly   respectively.


 


\textbf{Answering Causal Queries with a Trained \DCM.}  We now describe how a trained \DCM model can be used for (approximately) answering causal queries. Answering observational and interventional queries require sampling from the observational and the interventional distribution respectively. With counterfactuals, a query is at the unit level, where the structural assignments are changed, but the exogenous noise is identical to that of the observed datum.
% For interventional and counterfactual queries, consider a set of intervened variables $X_{\cI} \subseteq \mathbf{X}$ (for $\cI \subseteq [K]$)  and values $\gamma \in \R^{|\cI|}$, where $\doo(X_\cI:=\gamma)\coloneqq\{\doo(X_i:=\gamma_i)\}_{i\in\cI}$. 

\textbf{(a) Generating Samples for Observational/Interventional Queries.} Samples from a \DCM model that approximates the interventional distribution $p(\mathbf{X}\mid \doo(X_\cI:=\gamma))$ can be generated as follows. For an intervened node $i$ with intervention $\gamma_i$, the sampled value is always the intervention value, therefore we generate $\hat X_i:=\gamma_i$. 
% For root nodes, we sample $\hat X_i$ from the empirical distribution of the training set. 
For a non-intervened node $i$, assume by induction we have the generated parent values $\hat X_{\pa_i}$. To generate $\hat X_i$, we first sample the latent vector $Z_i\sim\cN(0,I_{d_i})$ where $d_i$ is the dimension of $X_i$. Then taking $Z_i$ as the noise for node $i$, we compute $\hat X_i:=\dec_i(Z_i,\hat X_{\pa_i})$ as the generated sample value for node $i$. This value $\hat X_i$ is then used as the parent value for the children of node $i$. Samples from a \DCM model that approximates the observational distribution $p(\mathbf{X})$ can be generated by setting $\cI=\emptyset$ (see Algorithm~\ref{algo: cdm intervention sampling}).

\begin{algorithm}[!h]
    \caption{Observational/Interventional Sampling}
    \label{algo: cdm intervention sampling}
    \textbf{Input:} Intervention set $\cI$ with values $\gamma$ ($I = \emptyset$ for observational sampling)
    \begin{algorithmic}[1]
        \FOR{$i=1,\ldots,K$} %\hfill\COMMENT{in topological order}
            \STATE $Z_i \sim\cN(0,I_{d_i})$
            \IF{$i\in \cI$}
            \STATE $\hat X_i \leftarrow \gamma_i$
            % \ELSIF{$i$ is a root node}
            % \STATE $\hat X_i\sim \mathcal{E}_i$ where $\mathcal{E}_i$ is the empirical distribution of the node $X_i$
            \ELSE
            \STATE $\hat X_i \leftarrow \dec_i(Z_i,\hat X_{\pa_i})$
            \ENDIF
        \ENDFOR
    \STATE Return $\hat X := (\hat X_1,\dots,\hat X_K)$
    \end{algorithmic}
\end{algorithm}




\begin{algorithm}[!h]
    \caption{Counterfactual Inference}
    \label{algo: DCM counterfactual inference}
    \textbf{Input:} Intervention set $\cI$ with values $\gamma$, factual sample~$x^\fact := (x_1^\fact,\dots,x_K^\fact)$
    \begin{algorithmic}[1]
     \FOR{$i=1,\ldots,K$} 
        \IF{$i\in \cI$}
            \STATE $\hat x^\cf_i \leftarrow \gamma_i$
            \ELSIF{$i$ is not a descendant of any node in $\cI$}
            \STATE $\hat x^\cf_i \leftarrow x^\fact_i$
            \ELSE
            \STATE  $z^\fact_i\leftarrow \enc_i(x^\fact_i,x_{\pa_i}^\fact)$ \hfill \COMMENT{abduction step}
            \STATE $\hat x^\cf_i \leftarrow \dec_i(z_i^\fact,\hat x_{\pa_i})$ \hfill\COMMENT{action and prediction}
            \ENDIF
        \ENDFOR
     \STATE Return $\hat x^\cf := (\hat x^\cf_1,\dots,\hat x^\cf_K)$
    \end{algorithmic}
\end{algorithm}

\textbf{(b) Counterfactual Queries.} 
Consider a factual observation $x^\fact:=(x_1^\fact,\dots,x_K^\fact)$ and interventions on a set of nodes $\cI$ with values $\gamma$. We use a \DCM model to construct a counterfactual estimate $\hat{x}^\cf$ as follows. The counterfactual estimate only differs from the factual value on intervened nodes or descendants of an intervened node. Similarly to interventional queries, for each intervened node $i \in \cI$, $\hat x_i^\cf:=\gamma_i$. For each non-intervened node $i$ that is a descendant of any intervened node, assume by induction that we have the generated counterfactual estimates $\hat x_{\pa_i}^\cf$. To obtain $\hat x_i^\cf$, we first define the estimated factual noise as $\hat z_i^\fact:=\enc_i(x_i^\fact, x_{\pa_i}^\fact)$. Then we  generate our counterfactual estimate by using $\hat z_i^\fact$ as the noise for node $i$, by decoding, $\hat x_i^\cf := \dec_i(\hat z_i^\fact,\hat x_{\pa_i}^\cf)$ (see Algorithm \ref{algo: DCM counterfactual inference}). 

Note that with $x^\fact$, we assumed full observability,\!\footnote{This is a common assumption in literature also made in all the related work e.g.,~\citep{vaca,carefl,pawlowski2020deep}.} since because Algorithm \ref{algo: DCM counterfactual inference} produces a counterfactual estimate for each node. However, when intervening on $X_\cI$ and if the only quantity of interest is  counterfactual on some $X^\star$, then you only need factual samples from $\{X_i:X_i\text{ is on a path from } X_{\cI} \to X^\star\}$~\citep{sahanoise}. In practice, this could be further relaxed by imputing for missing data, which is beyond the scope of this work.
% \textcolor{blue}{However, if we are only interested in counterfactual estimate at some node $\hat X_i^\cf$, all we need is for $X^\fact$ to contain values of $X_i$ and its ancestors. }
% \marginpar{To check this, can we set $Z_i$'s to $I_{d_i}$?}
% \textcolor{blue}{However, as is evident from Algorithm \ref{algo: DCM counterfactual inference},  if we are only interested in counterfactual estimate at some node $\hat X_i^\cf$, all we need is for $X^\fact$ to contain both $X_i^\fact$ and $X_{\pa_i}^\fact$ as we will see in the next section. In practice, even this could be relaxed by imputing for missing data, which is beyond the scope of this work.}
% \textcolor{red}{This does not seem to be true, you need $X_i^\fact$, $X_{\pa_i}^\fact$, and $\hat X_{\pa_i}$, which implicitly contains all of the upstream values as well.}
% \marginpar{How about this?}



==> tex_files/prelims_icml_workshop.tex <==

\textbf{Notation.} To distinguish random variables from their instantiation, we represent the former with capital letters and the latter with the corresponding lowercase letters.
To distinguish between the nodes in the causal graph and diffusion random variables, we use subscripts to denote graph nodes. Let $[n]:=\{1,\ldots,n\}$. 

\textbf{Structural Causal Models.} Consider a directed acyclic graph (DAG) $\cG$ with nodes $\{1,\dots,K\}$ in a topologically sorted order, where a node $i$ is represented by a (random) variable $X_i$ in some generic space $\cX_i \subset \R^{d_i}$. Let $\pa_i$ be the parents of node $i$ in $\cG$ and let $X_{\pa_i}\coloneqq \{X_j\}_{j\in\pa_i}$ be the variables of the parents of node $i$. 
% Without loss of generalization, assume the nodes $\cV$ are i. 
A structural causal model $\cM$ describes the relationship between an observed/endogenous node $i$ and its causal parents.
Formally, an SCM $\cM := (\mathbf{F},p(\mathbf{U}))$ determines how a set of $K$ endogenous random variables $\mathbf{X} := \{X_1,\dots,X_K\}$ is generated from a set of exogenous random variables $\mathbf{U} := \{U_1,\dots,U_K\}$ with prior distribution $p(\mathbf{U})$
via a set of structural equations, $\mathbf{F}:=(f_1,\ldots,f_K)$ where $X_i := f_i(X_{\pa_i},U_i)$ for $i \in [K]$. Throughout this paper, we assume that the unobserved random variables are jointly independent (Markovian SCM), and the DAG $\cG$ is the graph induced by~$\cM$.  Every SCM $\cM$ entails a unique joint observational distribution satisfying the causal Markov assumption: $p(\mathbf{X}) = \prod_{i=1}^K p(X_i\mid X_{\pa_i})$.
% where each conditional distribution $p(X_i\mid X_{\pa_i})$ is determined by the corresponding equation and noise distribution.

% PG(x), satisfying the causal Markov assumption: each variable is independent of its non-effects given
% its direct causes. It therefore factorises as PG(x) = QK
% k=1 PG(xk |pak), where  [1].

% implying $X_i$ is solely a function of its direct parents and its exogenous variable $U_i$, inducing a joint distribution: $p(X_1,\ldots,X_K) = \prod_{i=1}^K p(X_i\mid X_{\pa_i})$.
 
Structural causal models address Pearl's causal hierarchy (or ``ladder of causation''), which consists of three ``layers'' of causal queries in increasing complexity \citep{Pearl}: observational (or associational), interventional, and counterfactual. 
% In simple terms, observational queries relate to observing and recording events, interventional queries relate to intervening or acting to bring about change, and counterfactual queries involve reasoning, imagining, or understanding hypothetical scenarios. 
As an example, an interventional query can be formulated as ``What will be the effect on the population $\mathbf{X}$, if a variable $X_i$ is assigned a fixed value $\gamma_i$?'' The do-operator $\doo(X_i:=\gamma_i)$ represents the effect of setting variable $X_i$ to $\gamma_i$. Note that our proposed framework allows for more general sets of interventions as well, such as interventions on multiple variables denoted as $\doo(X_\cI:=\gamma)$ (where $\cI\subseteq [K]$, $X_{\cI} := (X_i)_{i \in \cI}$, $\gamma \in \R^{|\cI|}$). An intervention operation,  $\doo(X_\cI:=\gamma)$,  transforms the original joint distribution into an interventional distribution denoted by $p(\mathbf{X} \mid \doo(X_\cI:=\gamma))$.
On the other hand, a counterfactual query can be framed as ``What would have been the outcome of a particular factual sample $x^\fact:=(x_1^\fact,\dots,x_K^\fact)$, if the value of $X_\cI$ had been set to $\gamma$?''. Counterfactual estimation may be performed through the three-step procedure of 1) abduction: estimation of the exogenous noise $U$, 2) action: intervene $\doo(X_\cI:=\gamma)$, and 3) prediction: estimating $x^{\text{CF}}$ using the abducted noise and intervention values. 

% 


% \textbf{Observational Queries}


% \begin{CompactEnumerate}
%     \item \textbf{Associational/Observational Queries:} Evaluate the observational distribution $p(X_1,\ldots,X_K)$.
%     \item \textbf{Interventional Queries:} Evaluate the interventional distribution $p(\mathbf{X} \mid \doo(X_\cI:=\gamma))$.
%     \item \textbf{Counterfactual Queries:} Given a factual sample $X^{\text{F}}$, evaluate the counterfactual distribution $p(X^{\text{CF}} \mid X^{\text{F}},\doo(X_\cI:=\gamma))$.
% \end{CompactEnumerate}
% For the rest of this paper, we use `observational queries' to also represent `associational queries', since they are sampling the observational distribution. 

 % This may be interpreted as removing all incoming edges to node $i$ and setting $X_i=\gamma_i$, therefore only affecting descendants of node $i$.  Interventional queries address the distribution of $X$ when a subset is set to $\gamma$, notably different than conditioning on $X_\cI=\gamma$. Counterfactual queries address the distribution of $X^{\text{CF}}$ for a fixed factual observation $X^{\text{F}}$ when a subset is intervened to $\gamma$. 

\textbf{Diffusion Models.} Given data from distribution $X^0\sim Q$, the objective of diffusion models is to construct an efficiently sampleable distribution approximating  $Q$. Denoising diffusion probabilistic models (DDPMs) \citep{sohl-dickstein, ddpm} accomplish this by introducing a forward noising process that adds isotropic Gaussian noise at each time step and a learned reverse denoising process. A common representation of diffusion models is a fixed Markov chain that adds Gaussian noise with variances $\beta_1,\ldots,\beta_T\in (0,1)$, generating latent variables $X^1,\ldots,X^T$,
\begin{align*}
 q(X^t\mid x^{t-1})&= \cN(X^t; \sqrt{1-\beta_t}x^{t-1},\beta_t I)\\
 q(X^t\mid x^0)&=\cN(X^t; \sqrt{\alpha_t}x^{0},(1-\alpha_t)I)
\end{align*}
where $\alpha_t:=\prod_{i=1}^t (1-\beta_i)$.  Here, $T \in \mathbb{Z}^+$, and $t \in \{0,\dots,T\}$ denotes the time index. 

By choosing sufficiently large $T$ and $\alpha_t$ that converge to $0$, we have $X^T$ is distributed as an isotropic Gaussian distribution. The learned reverse diffusion process attempts to approximate the intractable $q(X^{t-1}\mid x^t)$ 
using a neural network and is defined as a Markov chain with Gaussian transitions,
\begin{align*}
    p_\theta(X^{t-1}\mid x^t) = \cN(X^{t-1};\mu_\theta(x^t,t),\Sigma_\theta(x^t,t)).
\end{align*}

Rather than predicting $\mu_\theta$ directly, the network could instead predict the Gaussian noise $\ep$ from $x^t=\sqrt{\alpha_t}x^0+\sqrt{1-\alpha_t} \ep$. \citet{ddpm} found that modeling $\ep$ instead of $\mu_\theta$, fixing $\Sigma_\theta$, and using the following reweighted loss function
\begin{align}\label{eq: simple objective}
   \mathbb{E}_{\mathrel{\substack{t\sim \mathrm{Unif}\{[T]\}\\X^0\sim Q\\ \ep\sim \cN(0,I)}}}[ \|\ep-\ep_\theta(\sqrt{\alpha_t}X^0+\sqrt{1-\alpha_t} \ep,t)\|^2],
\end{align}
works well empirically. We also utilize this loss function in our training.

\citet{ddim} introduce a richer family of distributions, where it is possible to use a pretrained DDPM model to obtain a deterministic sample given noise $X^T$, known as the denoising diffusion implicit model (DDIM), with \textit{reverse implicit diffusion process}
\begin{align}
\begin{split}\label{eq: ddim reverse}
     X^{t-1} &\coloneqq \sqrt{ \frac{\alpha_{t-1}}{\alpha_t}}X^t - \ep_\theta(X^t,t)\;\cdot \\
     &\quad \left(\sqrt{\alpha_{t-1}(1-\alpha_{t})/\alpha_t}-\sqrt{1-\alpha_{t-1}}\right).
     \end{split}
\end{align}
Note that the $X^t$ here is deterministic. We also use a \textit{forward implicit diffusion process} introduced by \citet{ddim}, derived from rewriting the DDIM process Eq.\ \eqref{eq: ddim reverse} as an ordinary differential equation (ODE) and considering the Euler method approximation in the forward direction to obtain 
\begin{align}\label{eq: forward implicit diffusion}
\begin{split}
    X^{t+1} &\coloneqq  \sqrt{\frac{\alpha_{t+1}}{\alpha_t}}X^t + \ep_\theta(X^t,t)\; \cdot \\
    &\quad \left(\sqrt{1-\alpha_{t+1}}-\sqrt{\alpha_{t+1}(1-\alpha_t)/\alpha_t}\right).
\end{split}
\end{align}
We utilize the DDIM framework in this work, in particular Eqs.\ \eqref{eq: forward implicit diffusion} and \eqref{eq: ddim reverse} will define the encoding (forward) and decoding (reverse) processes.


==> tex_files/pseudocodes.tex <==


\begin{algorithm}[!h]
    \caption{$\enc_i(X_i,X_{\pa_i})$}
    \label{algo: DCM encoding}
    \textbf{Input:}  $X_i$, $X_{\pa_i}$
    \begin{algorithmic}[1]
      \STATE $Z_i^0\leftarrow X_i$ 
        \FOR{$t=0,\ldots,T-1$}
           \STATE 
$Z^{t+1}_i \leftarrow\sqrt{\frac{\alpha_{t+1}}{\alpha_t}}Z^t_i + \ep_\theta^i(Z^t_i,X_{\pa_i},t)\left(\sqrt{1-\alpha_{t+1}}-\sqrt{\frac{\alpha_{t+1}(1-\alpha_t)}{\alpha_t}}\right)$
        \ENDFOR
    \STATE Return $Z_i\coloneqq Z_i^T$
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[!h]
    \caption{$\dec_i(Z_i,X_{\pa_i})$}
    \label{algo: DCM decoding}
    \textbf{Input:}  $Z_i$, $X_{\pa_i}$
    \begin{algorithmic}[1]
     
      \STATE $\hat X^T\leftarrow Z_i$
        \FOR{$t=T,\ldots,1$}
         
\STATE 
$\hat X^{t-1}_i \leftarrow\sqrt{ \frac{\alpha_{t-1}}{\alpha_t}}\hat X^t_i -\ep_\theta^i( \hat X_i^t,X_{\pa_i},t)  \left(\sqrt{\frac{\alpha_{t-1}(1-\alpha_{t})}{\alpha_t}}-\sqrt{1-\alpha_{t-1}}\right)$
              
    \ENDFOR    
    \STATE Return $\hat X_i\coloneqq \hat X_i^0$
    \end{algorithmic}
\end{algorithm}

==> tex_files/theory_amlc.tex <==
We now establish {\em sufficient} conditions under which the counterfactual estimation error can be bounded. In fact, the results in this section not only hold for diffusion models, but to a more general setting of conditional latent variable models satisfying certain properties. 
% We define a latent variable model using an encoder ($g()$) and decoder function ($h()$).

We focus on learning a single conditional latent variable model for an endogenous node $X_i$, given its parents $X_{\pa_i}$, as the models learned for different endogenous nodes do not affect each other. Since the choice of node $i$ plays no role, we drop the subscript $i$ in the following and refer to the node of interest as $X$, its causal parents as $X_\pa$, its corresponding exogenous variables as $U$, and its structural equation as $X:=f(X_\pa,U)$. Let the encoding function $g:\cX \times \cX_{\pa} \to \cZ$  and the decoding function $h: \cZ\times \cX_{\pa} \to \cX$, where $\cZ$ is the latent space. In the \DCM context, the functions $g$ and $h$ correspond to $\enc$ and $\dec$ functions, respectively. 

It is well-known that that certain counterfactual queries are not identifiable from observational data without making assumptions on the functional relationships, even under causal sufficiency~\citep{pearl2009causal}. Consequently, recent research has been directed towards understanding the conditions under which identifiability results can be obtained~\citep{lu2020sample,nasr2023counterfactual,nasr2023}. Assumption 2 of our Theorem~\ref{thm: cf theory}, ensures that the true counterfactual outcome is identifiable, see e.g.,~\citep[Theorem 1]{lu2020sample} or~\citep[Theorem 5]{nasr2023counterfactual}. In the context of learned structural causal models to determine whether a given counterfactual query can be answered with sufficient accuracy, requires also assumptions on the learned SCM, e.g., encoder and decoder in this case.

% , as well as the functional relationships between the variables in the model. 

% which are learned from data using machine learning methods, the goal is to determine whether a given counterfactual query can be answered with sufficient accuracy and under what conditions. This involves understanding the assumptions and limitations of the learned SCM, as well as the functional relationships between the variables in the model. 


% We utilize a similar assumption on $f$ as (see ), under which the 
% which does not require some of the bijectiveness assumptions utilized in~\citep{nasr2023counterfactual,nasr2023}.

% As learning the generation function of $X_i$ does not have any effect on learning the generation
% function of Vj for , we focus on learning the generation function of a single node Vi henceforth. 


% In the context of learned structural causal models (SCMs), which are learned from data using machine learning methods, the goal is to determine whether a given counterfactual query can be answered with sufficient accuracy and under what conditions. This involves understanding the assumptions and limitations of the learned SCM, as well as the functional relationships between the variables in the model. 


Our first result presents sufficient conditions on the latent variable encoding function and the structural equation under which we can recover latent exogenous variable up to a (possibly nonlinear) invertible function. For simplicity, we start with a one-dimensional exogenous noise $U$ and variable $X \in \cX \subset \R$. We provide a similar theorem for the multivariate case where $X \in \R^m$ for $m\ge 3$ in Theorem \ref{thm: multivariate cf theory} in the Appendix~\ref{app: multivariate theory} with a stronger assumption on the Jacobian of $f$ and $g$.

\begin{restatable}{theorem}{first}
\label{thm: cf theory}
Assume for $X \in \cX\subset \R$ and exogenous noise $U\sim \mathrm{Unif}[0,1]$, $X$ satisfies the structural equation: $X:=f(X_{\pa},U)$, where $X_\pa \in \cX_\pa \subset \R^d$ are the parents of node $X$ and $U\indep X_\pa$. Consider an encoder-decoder model with encoding function $g:\cX\times \cX_{\pa} \to \cZ$ and decoding function $h: \cZ\times \cX_{\pa} \to \cX$, 
$    Z:=g(X,X_{\pa}), \quad \hat X:=h(Z,X_{\pa})$.
Assume the following conditions:
\begin{CompactEnumerate}   
    \item The encoding is independent of the parent values, $g(X,X_{\pa})\indep X_{\pa}.$ 
    \item The structural equation $f$ is differentiable and strictly increasing with respect to $U$. 

    \item The encoding $g$ is invertible and differentiable with respect to $X$.
\end{CompactEnumerate}
Then, $g(X,X_\pa) = \tilde q (U)$ for an invertible function $\tilde q$.
\end{restatable} 
In Appendix~\ref{app: proofs}, we discuss the assumptions underlying Theorem~\ref{thm: cf theory}, and its consequences for estimating counterfactual error. All proofs are also collected in Appendix \ref{app: proofs}. 



% Consider a node $i$ (represented by $X_i \in \cX_i$) in the causal graph and its parents (represented by $X_{\pa_i} \in \cX_{\pa_i}$). 
% \noindent\textbf{Discussion on Assumptions Underlying Theorem~\ref{thm: cf theory}.}

% \textbf{(1)} Assumption 1 of independence between the encoding and the parent values may appear strong, but is in fact often valid. For example, in the additive noise setting with $X:=f(X_\pa)+U$ where $X_\pa$ and $U$ are independent, if the fitted model $\hat f \equiv f$, then the encoder $g(X,X_\pa)=X-\hat f(X_\pa)=U$ and by definition $U$ is independent of $X_\pa$.\footnote{In general, if we have a good approximation $f$ by some $\hat{f}$, then the encoding $g(X,X_\pa)=X-\hat{f}(X_\pa)$ would be close to $U$, as also noted by~\citep{hoyer2008nonlinear}.} The same assumption also appears in other related  results on counterfactual identifiability in bijective SCMs, see, e.g.,~\citep[Theorem 5.3]{nasr2023} and proof of Theorem 5 in~\citep{nasr2023counterfactual}. 
% We conduct empirical tests to further confirm this assumption by examining the dependence between the parents and encoding values. Our experimental results show that DCMs consistently fail to reject the null hypothesis of independence. This implies that independent encodings can be found in practice. We provide the details of these experiments in Appendix~\ref{app: independence exp}.\!\footnote{To encourage independence, one could also modify the original diffusion model training objective to add a Hilbert-Schmidt independence criterion (HSIC) \citep{HSIC} regularization term. Our experiments did not show a clear benefit of using this modified objective, and we leave further investigation here for future work.}.

% % One may measure the dependence between encodings and parent values on training or hold out data to verify the claim, for example through measuring the Hilbert-Schmidt independence criterion (HSIC) \citep{HSIC}. The heuristic of minimizing the dependence between regressors and residuals has been explored \citep{regression_dep_min}; our theoretical results independently motivate this heuristic \footnote{To encourage independence, one could also modify the original diffusion model training objective to add an HSIC regularization term. Our experiments did not show a clear benefit of using this modified objective, and we leave further investigation here for future work.}. 

% \textbf{(2)} Assumption 2 is always satisfied under the additive noise model (i.e.,  $X:=f(X_{\pa})+U$) and post non-linear models \citep{zhang2012identifiability}. Again, the recent results about counterfactual identifiability, e.g.,~\citep[Theorem 5]{nasr2023counterfactual} and~\citep[Theorem 1]{lu2020sample}, also utilize the same assumption. 
% % \textcolor{blue}{Did not follow:}The generalizability of the noise $U$ allows for common noise distributions, such as additive Gaussian noise.

% % \textbf{(3)} From the second assumption that the structural equation $X:=f(X_{\pa},U)$ is invertible with respect to $U$ in \Cref{thm: cf theory,thm: multivariate cf theory}, this suggests that our latent variable should be of equal dimension to the $X$ we are modeling. While some autoencoder models decrease the latent dimension with respect to the input, diffusion models retain the same dimension between $X$ and $U$ making them amenable to the above analysis.

% % \textbf{(4)} 
% \textbf{(3)} We may consider transformations of the uniform noise $U$ to obtain other settings, for example additive Gaussian noise. 
% % The only assumptions on the noise are independence from parents and the second assumption, stating, $f$ is  differentiable and strictly increasing with respect to $U$. 
% For a continuous random variable $U'$ with invertible CDF $F$ and the structural equation $f(\cdot,F(\cdot))$, we have $U'\stackrel{d}{=}F^{-1}(U)$ and the results similarly hold.


% % Finally, while these conditions are needed for our proof, in practice even under some violations,  our \DCM approach provides good empirical performance, suggesting the possibility of further refinement of the theorem statement.


% We now discuss some consequences of Theorem~\ref{thm: cf theory} for estimating counterfactual outcomes.

% % We now discuss two consequences for counterfactual identifiability and estimation error.
% \noindent\textbf{1. Perfect Estimation.} Using~\cref{thm: cf theory}, we now look at a condition under which the counterfactual estimate produced by the encoder-decoder model matches the true counterfactual outcome.\footnote{Note that identifiability of
% the counterfactual outcomes, does not require identifiability of the SCM.}. 
% The idea here been, if no information is lost in the encoding and decoding steps, i.e., $h(g(X,X_\pa),X_\pa) = X$, and assuming~\cref{thm: cf theory}  ($g(X,X_\pa) = \tilde q(U)$), we have $h(\tilde q (U),X_\pa) = X = f(X_\pa,\tilde q^{-1}(U))$. This means that in the abduction step, the encoder-decoder model could recover $\tilde q(U)$, but in the prediction step with, it first applies the inverse of $\tilde q$ to the recovered exogenous variable, and then $f$. Thus, the counterfactual estimate equals the true counterfactual outcome.


% \begin{restatable}{corollary}{iden} \label{cor: iden}
% Assume the conditions of~\cref{thm: cf theory}. Furthermore, assume the encoder-decoder model pair $(g,h)$ satisfies: $h(g(X,X_{\pa}),X_{\pa}) = X$.
% Consider a factual sample pair $x^\fact:=(x,x_\pa)$  where $x:=f(x_\pa,u)$ and an intervention $\doo(X_{\pa}:=\gamma)$. Then, the counterfactual estimate, given by $h(g(x,x_\pa),\gamma)$ matches the true counterfactual outcome $x^\cf := f(\gamma,u)$.
% \end{restatable}
% % \textcolor{red}{Where is corollary 1?}
% % \textcolor{red}{reference to proof is missing}
% % where we use a recent result of~\citet{nasr2023counterfactual}. It is important to show that the counterfactual outcome is identifiable. 

% % \begin{theorem}[Restated Theorem 4 of~\citet{nasr2023counterfactual}] \label{thm: iden}
% % Using a model class for learning a bijective structural equation $f$ leads to identifiable counterfactual estimates if all the models in that class that fit the observational conditional distribution, recover the same exogenous variable up to a nonlinear
% % invertible indeterminacy
% % \end{theorem}
% % Putting together Theorems~\ref{thm: cf theory} and~\ref{thm: iden}, we get the following result.
% \noindent\textbf{Comparison with Recent Related Work.} Recent studies by~\citet{nasr2023counterfactual} and~\citet{nasr2023} have explored the problem of estimating counterfactual outcomes with learned SCMs. In particular,~\citet{nasr2023counterfactual} consider a setting where the SCM $X:=f(X_\pa,U)$ is learned with a {\em bijective} (deep conditional generative) model $\hat{f}(X_\pa,\hat{U})$~\citep[Theorem 5]{nasr2023counterfactual}).~\citet[Theorem 5.3]{nasr2023} considered a closely related problem of learning a ground-truth bijective SCM.
% The conditions underlying ours and these results are not directly comparable because, unlike our setup, they do not explicitly consider an encoder-decoder model.  Our results provide precise conditions on the encoder $g$ and decoder $h$ for recovering the correct counterfactual outcome, and we can extend these results to obtain counterfactual estimation error bounds under relaxed assumptions, a problem that has not been addressed previously.



% % \textcolor{blue}{Explain difference between~\cref{thm: cf theory} and Theorem 5 of~\citep{nasr2023counterfactual}.}



% \noindent\textbf{2. Estimation Error.}
% Another consequence of Theorem \ref{thm: cf theory} is that it can bound the counterfactual error in terms of the reconstruction error of the encoder-decoder model. Informally, the following corollary shows that if the reconstruction $h(g(X,X_{\pa}),X_{\pa})$ is ``close'' to $X$ (measured under some metric $d(\cdot,\cdot)$), then such encoder-decoder models can provide ``good'' counterfactual estimates.  To the best of our knowledge, this is the first result that establishes a bound on the counterfactual error in relation to the reconstruction error of these encoder-decoder models.
% \begin{restatable}{corollary}{est} \label{cor: est}
% Let $\gamma \ge 0$. Assume the conditions of~\cref{thm: cf theory}.  Furthermore, assume the encoder-decoder model pair $(g,h)$ under some metric $d$ (e.g., $\|\cdot \|_2$), has reconstruction error less than $\tau$: $d(h(g(X,X_{\pa}),X_{\pa}),X)\le \tau$. Consider a factual sample pair $x^\fact:=(x,x_\pa)$  where $x:=f(x_\pa,u)$ and an intervention $\doo(X_{\pa}:=\gamma)$. Then, the error between the true counterfactual $x^\cf := f(\gamma,u)$ and counterfactual estimate given by $h(g(x,x_\pa),\gamma)$ is at most $\tau$, i.e., $d(h(g(x,x_\pa),\gamma), x^\cf)\le \tau$.
% \end{restatable}
% % \textcolor{red}{Reference to proof is missing}
% The above result suggests that the reconstruction error can serve as an estimate for the counterfactual error. While the true value of $\tau$ is unknown, we may compute a reasonable bound by computing the reconstruction error over the dataset. 


% % \begin{restatable}{theorem}{first}
% % \label{thm: cf theory}
% % Assume for $X \in \cX\subset \R$ and exogenous noise $U\sim \mathrm{Unif}[0,1]$, $X$ satisfies the structural equation: $X=f(X_{\pa},U)$, where $X_\pa \in \cX_\pa \subset \R^d$ are the parents of node $X$ and $U\indep X_\pa$. 

% % Consider an encoder-decoder model with encoding function $g:\cX\times \cX_{\pa} \to \cZ$ and decoding function $h: \cZ\times \cX_{\pa} \to \cX$, 
% % \begin{align*}
% %     Z=g(X,X_{\pa}), \quad \hat X=h(Z,X_{\pa}).
% % \end{align*}
% % Assume the following conditions are met:
% % \begin{enumerate}
% % \vspace*{-2ex}
% %     \item The encoding is independent from the parent values, $g(X,X_{\pa})\indep X_{\pa}.$ 
% %     \item Under some metric $d$ e.g., $\|\cdot \|_2$, the model has reconstruction error less than $\tau$,
% % \begin{align}\label{eq: reconstruction error}
% % d(h(g(X,X_{\pa}),X_{\pa}),X)\le \tau.
% % \end{align}
% %     \item The structural equation $f$ is invertible, differentiable, and increasing with respect to $U$.
% %     \item The encoding $g$ is invertible and differentiable with respect to $X$.
% % \end{enumerate}

% % Then for a pair $(x_\pa,u)$ and the factual sample $x=f(x_\pa,u)$, the noise $u$ is identifiable up to an invertible function. Furthermore for an intervention $\doo(X_{\pa}:=\gamma)$, the counterfactual estimate from the model of the true counterfactual $x^\cf = f(\gamma,u)$ using the factual $x=f(x_\pa,u)$ has estimation error at most $\tau$: $d(h(g(x,x_\pa),\gamma), x^\cf)\le \tau$.
% % \end{restatable} 

